NG-Scope: Fine-Grained Telemetry for NextG Cellular Networks

Accurate and highly-granular channel capacity telemetry of the cellular last hop is crucial for the effective operation of transport layer protocols and cutting-edge applications, such as video on demand and videotelephony. This paper presents the design, implementation, and experimental performance evaluation of NG-Scope, the first such telemetry tool able to fuse physical-layer channel occupancy readings from the cellular control channel with higher-layer packet arrival statistics and make accurate capacity estimates. NG-Scope handles the latest cellular innovations, such as when multiple base stations aggregate their signals together to serve mobile users. End-to-end experiments in a commercial cellular network demonstrate that wireless capacity varies significantly with channel quality, mobility, competing traffic within each cell, and the number of aggregated cells. Our experiments demonstrate significantly improved cell load estimation accuracy, missing the detection of less than 1% of data capacity overall, a reduction of 82% compared to OWL, the state-of-the-art in cellular monitoring. Further experiments show that MobileInsight-based CLAW has a root-mean-squared capacity error of 30.5 Mbit/s, which is 3.3x larger than NG-Scope (9.2 Mbit/s)

==> Abstract.tex <==
Accurate, highly-granular measurement of channel capacity of the 
cellular last hop is crucial for 
the effective operation of transport layer protocols and
cutting edge applications, such as video on demand and video telephony.  
This paper presents the design, implementation,
and experimental performance evaluation of \systemname{}, the first
cellular capacity monitor able to
fuse physical-layer channel occupancy readings from the cellular
control channel with higher-layer packet arrival statistics and
make accurate capacity estimates when 
multiple base stations aggregate together, to serve a single mobile user. 
End-to-end experiments using \systemname{} in a commercial cellular network 
demonstrate that wireless capacity varies significantly 
with channel quality, mobility, competing traffic within each cell 
and the number of aggregated cells.
Experiments demonstrate significantly improved cell load estimation accuracy, 
missing detection of less than 1\% of data capacity overall,
a reduction of 82\% compared to OWL~\cite{OWL}, 
the state-of-the-art in cellular monitoring.
Further experiments show that 
MobileInsight\hyp{}based \cite{MobileInsight}
CLAW~\cite{CLAW} has a root\hyp{}mean\hyp{}squared capacity error
of 30.5~Mbit/s, which is 3.3$\times$ larger than \systemname{} (9.2~Mbit/s).



%comparing with the detection results of \systemname{},
%\textcolor{red}{More experimental results comparing with CLAW~\cite{CLAW} and BurstTracker~\cite{BurstTracker} to be updated}
%\textcolor{red}{the amount by which you reduce false positive and misses doesn’t matter if the others are accurate already.  You need more numbers at the end of the abstract and more head-to-head numbers that compare accuracy.}

%Further experiments demonstrate that \systemname{} is able to track capacity 
%variations with millisecond level granularity, enabling agile congestion control.


% We observe the high packet error rate (7\% to 12\%) in LTE network 
% which are affected by packet size and UE mobility. We demonstrate that the mobility,
% the competing traffic and the carrier aggregation of a LTE link varies significantly, 
% resulting in large fluctuation of link capacity. 

% We have implemented \systemname{} on multiple USRP software defined radio platforms, host PCs, 
% and a mobile phone in a design that synchronizes and fuses information from the USRPs with the mobile phone.  
% Our performance evaluation investigates the accuracy of \systemnames{} control channel decoder,
% demonstrating a reduction in missed control messages to 0.8\% (a 82\% reduction over OWL). 
% \systemname{} also reduces the rate of false positives (detection of nonexistent control messages) 
% by 92\% compared to OWL.



==> Append.tex <==
\section{Appendix: Responds to reviewers' revision requests}

\noindent
\textbf{Comment: Concerns on time complexity and PC-based evaluation.} 
It is a major concern from all the reviewers. 
The PoC and experiments in this paper were implemented and evaluated on a PC instead of a mobile UE. 
All the results were collected based on strong computational capacity provided by the PC. 
We all concerned if computational requirements of the proposed algorithms 
could be met by future generations of mobile devices. 
The experiments of CPU load on an Intel Xeon don't shed insight into 
how much computing would be needed on the UE to run these algorithms. 
It is suggested that authors can have discussions on that as well as time complexity analysis for the proposed algorithms.

\noindent
\textbf{Response:} 
We agree with the reviewer that a pure PC based computational overhead evaluation 
is not enough to demonstrate the feasibility of \systemname{}.
We conduct theoretical analysis on the \systemnames{} computational overhead 
and find the the overhead is determined by the number of convolutional decoding attempts 
\systemname{} needs to perform when decoding each subframe. 
We therefore measured the exact number of decoding attempts 
\systemname{} performs when decoding the control channel of a base station in real time,
the results are given in Figure~\ref{fig:nof_decode}.
We also compare such a number with a legacy mobile phone decoding its own control message 
and the result is that \systemname{} only introduces around 1$\times$ more decoding attempts. 
Please refer to Section~\S\ref{s:comp} for the detailed analysis. 
\vspace{0.3cm}

\noindent
\textbf{Comment: App/End-To-End level performance evaluation} 
The paper could be stronger with some experimental evidence that the capabilities provided by LTScope 
can be further used to improve some aspect of end-to-end performance or real-world application. 
In other words, it would be helpful to emulate some application (e.g., video streaming) and demonstrate 
how LTScope helps improve channel capacity estimation and in turn bit rate adaptation? 
The comparison to other works (OWL, CLAW and BurstTracker) using an application might also help tackle the ground truth challenge.

\noindent
\textbf{Response:} 
We want to thanks the reviewer for the advice. 
We build a congestion control algorithm that takes the fine-grain capacity estimation reported by \systemname{} as input 
and compare the performance of such a algorithm with seven state-of-the-art congestion control algorithms. 
Please refer to Section~S\ref{s:congestion} for more details about the comparison. 
\vspace{0.3cm}

\noindent
\textbf{Comment: Practical concerns on applicability.}
It would be more than interesting to see discussions on some practical concerns such as 
what’s the desirable frequency designed for updating capacity estimation results? 
how fast it can support for those updates, and how to update, threshold based approach or update upon any difference and so on. 

\noindent
\textbf{Response:}
We want to thanks the reviewer for pointing out one missing piece of design in our previous version of manuscript. 
\systemname{} is able to update the capacity at a frequency every one millisecond. 
We introduce the details of calculating the capacity in Figure~\ref{fig:cap_update} and its corresponding text. 
Please refer to Section~\S\ref{s:imp} for more details. 

Updating the capacity estimation every one millisecond is the maximum frequency \systemname{} is able to provide. 
The system still works at lower updating frequency, \eg, every 10~$ms$, 20~$ms$ or 50~$ms$. 
It is also possible for us to implement a middle layer atop of \systemname{}, 
which sends an update to the application when and only when the capacity variation 
since last update exceeds a threshold. 

We note that the desirable updating frequency should be determined by the applications. 
For example, congestion control algorithms update their actions upon every packet reception 
so that highest capacity updates provides them most up-to-date information for better decision. 
Video streaming applications, however, select resolution for video chunks and 
such a decision works for the whole period of time the user takes to download the chunk.
Therefore, video streaming does not require extremely high frequency rate updates, \eg, every one millisecond. 
We should adjust the updating frequency according to the characteristics of the application that leverages \systemname{}.
\vspace{0.3cm}


\noindent
\textbf{Comment: Clarification needed on some parts} 
It's better to have more explanation/clarification on some parts such as control message decoding: 
illustrative example would highly be helpful. 
How do you derive the C-RNTI using CRC and payload is not clear? 
Concept of aggregation level must better be explained. Fig.6 and Fig.7 need more explanation.

\noindent
\textbf{Response:} 
We would like to thank the reviewer for the suggestions. 
We add two new figures: Figure~\ref{fig:dci_encode} and \ref{fig:dci_cce}, 
and almost rewrite Section~\S\ref{s:decoder}: Control Message Decoder, 
to make the explanation of the decoding process clearer. 
We add a separate paragraph to explain how we derive the C-RNTI and payload. 
We hope our revision on the text could help to clarify the key concepts. 
\vspace{0.3cm}

\noindent
\textbf{Comment:} 
Section 3.3: "contains a transport layer packet with sequence number one." I'm confused by the statement. 
At least in TCP, bytes have sequence numbers, not packets. 
Second, is it always the case that one physical layer transport block corresponds to a transport layer "packet"? 
Doesn't that depend not only on the allocated PRB, but also on IP Path MTU discovery?

\noindent
\textbf{Response:}
Thanks for pointing out the confusing description. 
The sequence number is indeed confusing and not needed in this example. 
We just want to say the first packet and the second TCP or UDP packet the sender transmits. 
We have remove the concept of sequence number and revise the text to make it clearer. 
Figure~\ref{fig:tb_err_burst} is just an example of transmission error,
so it doesn't mean that it will always be the case that one physical 
layer transport block corresponds to a transport layer "packet". 
Their relationship indeed depends on the allocated PRB and MTU. 
\vspace{0.3cm}



%\noindent
%\textbf{Comment:} 
%The decoder finishes decoding within one millisecond (before the arrival of the next subframe) for 94 percent of subframes.": 
%I presume this is on the Intel Xeon machine that is used in section 5.2, 
%and not on the mobile device? 
%If so, can you comment on what it would take to translate some of this to cellular firmware 
%because I imagine the hardware for doing these computations is likely to be expensive
%
%\noindent
%\textbf{Response:}
%Thanks for asking such a question.
%The percentage of 94\% is measured when \systemname{} is running in real-time, decoding the control channel. 
%The implementation of \systemname{} is a single thread version. 
%To find out the exact reason why it appears, 
%in this round of revision, 
%we measure the time \systemnames{} Viterbi decoder takes to decode each control messages, 
%the results is plotted in Figure~\ref{fig:decode_time}.
%We also record how many decoding attempts \systemname{} takes 



%Initially, I implemented \systemname{} with a single-thread design and 
%I found that the time it takes to first separating the signal of one subframe and then decode
%is longer than one millisecond for many subfarmes. 
%cannot catch up with the 
%
%decoding speed cannot match with the speed of data coming i 
%I observed the phenomenon of using one decoder 
%\vspace{0.3cm}
%

\noindent
\textbf{Comment:} 
Section 5.1: While the direct comparison with OWL in terms of the number of control messages correctly decoded is helpful, 
it would have been more helpful to see an end to end experiment that 
quantifies the impact of the missed control messages on some application perceived performance.

\noindent
\textbf{Response:} 
Thanks for the suggestion. 
We provide such a comparison with a trace-driven emulation.
We randomly drop control messages before using it to the calculate the capacity at the TCP end-points.
We measure the performance of congestion control algorithms with different percentage of control message being dropped.
Please refer to Section~\S\ref{s:congestion} for more details. 

\vspace{0.3cm}

\noindent
\textbf{Comment:} 
Somehow, it was hard to appreciate the LTScope-ground truth based evaluation. 
May be there is some deeper intuition behind conducting the evaluation using this approach. 
If you can shed more light on why this is convincing, then that would be tremendously useful!

\noindent
\textbf{Response:} 
According to wireless theory, the signals at two locations is entirely independent from each other 
if the distance between these two locations is larger than half of the carrier wavelength.
The errors inside the bit stream demodulated from two independent signals should appear independently. 
For example, if we transmits 10 zeros: "0000000000" and 
get an bit error at the second bit in the first location, we will receive "0100000000". 
If the signal received from the second location is correlated with the first location, 
we have a very high chance to get a bit error at the second bit of the demodulated bit stream at the second location. 
But if the signals of two locations are independent each other, 
the bit errors also appear independently inside the demodulated bit stream.


The results after decoding the bit streams at above two locations are independent from each other. 
Supposing the chance of decoding successfully at each location is 95\%,
then we have $95\% \times 95\% = 90.25\%$ of chances that we will get the same correct result at both locations, 
which is a reasonably high chance. 
What will happen if the decoding is not successful? 
Actually, if the decoding is independent from each other, 
the chance that we get the exactly the same message 
after a inaccurate decoding is very close to zero, 
even when the input bit sequences have only 1 bit difference. 

Therefore, if we observe identical decoded messages from multiple independent locations, 
those messages are highly likely to be the correctly decoded messages, 
instead of two messages that are decoded incorrectly but just happened to be the same. 




==> Design.tex <==
\section{Design and Implementation}
\label{s:design}

We first introduce \systemnames{} architecture (\S\ref{s:sys_arch}). 
We then introduce the control channel decoder, which is a crucial component in our 
system (\S\ref{s:decoder}). Finally, we detail how we fuse
data collected from different base stations (\S\ref{s:fusion}), providing a 
a complete view of LTE communication to higher layers.

\subsection{System Architecture}  
\label{s:sys_arch}
With 

\systemname{} simultaneously decodes the control channels of multiple cell 
towers. For each cell tower, we use one off\hyp{}the\hyp{}shelf software 
defined radio, (the USRP~\cite{USRP}) as a front\hyp{}end to collect 
LTE signals, as shown in Figure~\ref{fig:system}. The signals 
the USRP collects are sent to the connected PC for decoding. 
\systemname{} imposes no limit on the number of cell towers that can be 
simultaneously monitored: we can extend the architecture to support 
more carriers by simply adding more PCs and software-defined radios. 
The actual number of carriers that should be monitored depends on the 
LTE standard, \eg 3GPP Release 13 allows aggregation of a maximum of 
32 carriers for a bandwidth of 640~MHz, and service provider implementation
also varies.  In the future, we envisage the entirety of \systemnames{}
functionality being implemented in custom LTE firmware and incorporated
into a UE via an over\hyp{}the\hyp{}air update.

\begin{figure}[thb]
    \centering
    \includegraphics[width=0.99\linewidth]{fig/system.pdf}
    \caption{\textit{\systemname{} architecture.} Each PC\hyp{}USRP 
    pair monitors one cell tower,
    while a pair designated \textit{master} collects decoded control 
    messages from others. 
    The master connects to the UE, which uses the commercial LTE network.}
    \label{fig:system}
\end{figure}


Among the PCs, we select one as the master, while the others function as slaves
and are connected to the master through a TCP connection. On each slave, we 
create three threads that work in parallel: a \textit{USRP handler} thread that
receives and buffers the IQ data from the software radio, a \textit{control channel 
decoder} thread that takes the buffered IQ data as input and decodes the control 
message contained therein, and a \textit{master handler} thread that sends the 
decoded control messages to the master. On the master, we create four threads. 
The USRP handler and control channel decoder work exactly the same as the ones 
on the slaves. The \textit{slave handler} thread receives control messages from
slaves. From Figure~\ref{fig:system}, we see that the master also connects to 
a commercial UE (a phone), which communicates with a remote server through the 
LTE network. The UE records packet reception statistics such as one\hyp{}way delay 
and reception time, and sends the resulting packet log to the master. Therefore,
we also create a \textit{UE handler} to receive the packet log from the mobile 
device for further analysis. \systemname{} combines and synchronizes the control
message data stream and the packet log. 
\begin{figure}[thb]
    \centering
    \includegraphics[width=0.99\linewidth]{fig/multi_thread.pdf}
    \caption{\textit{\systemname{} architecture.} Each PC\hyp{}USRP 
    pair monitors one cell tower,
    while a pair designated \textit{master} collects decoded control 
    messages from others. 
    The master connects to the UE, which uses the commercial LTE network.}
    \label{fig:system}
\end{figure}
\subsection{Control Channel Decoder}
\label{s:decoder}

In this section, we describe how \systemname{} decodes the LTE control
channel. We begin with the introduction of control information contained 
inside each control messages.  We then present a primer of LTE control 
channel decoding and at last describe \systemnames{} decoding algorithm.

\begin{table}[ht]
	\centering
	\begin{tabularx}{\linewidth}{@{}l@{\hspace*{2pt}}X@{}|@{\hspace*{1pt}}l@{\hspace*{2pt}}X@{}}
		\toprule
		\textbf{Field} & \textbf{Description} & \textbf{Field} & \textbf{Description} \\
		\hline
		\textsf{C-RNTI}& PHY ID& 
		\textsf{sfn}& Subframe index \\
		\textsf{MCS-1} &1$^{\textrm{st}}$\hyp{}stream MCS 
		    &\textsf{MCS-2} &2$^{\textrm{nd}}$\hyp{}stream MCS\\
		\textsf{nof\_prb}  &\# alloc.\ PRBs & \textsf{tbs}  &TB size (bits) \\ 
	    \textsf{ndi}  & New-data indicator & \textsf{harq} & HARQ process index \\
		\bottomrule
	\end{tabularx}
	\caption{Selected information fields conveyed by a control message (\textsf{MCS-2} is optional for MIMO modes only).}
	\label{t:DCI}
\end{table}
LTE defines 10 formats for control messages, depending on how much 
information  is delivered~\cite{TS213,TS212}. For example, control formats of LTE 
SISO transmissions only contain one MCS index. 
Table~\ref{t:DCI} summarizes control message information: 
the \textit{cell radio network temporary identifier} (\textsf{C-RNTI}) 
is the physical\hyp{}layer identifier for the receiver (user) of this control message. 
The subframe index (\textsf{sfn}) provides a timestamp of each
a message with a 1~ms resolution, as Figure~\ref{s:OFDMA} shows. 
The MCS index encodes the MCS as well as the number of spatial streams,
allowing us to
calculate how many data bits are transmitted in 
each transport block (\textsf{tbs}) using the MCS index 
and allocated PRBs (\textsf{nof\_prb}). 
LTE uses a non\hyp{}negligible portion of 
channel time to retransmit errored data (\S\ref{s:eval_reTx}), so  
we detect these retransmissions using the \textsf{new-data} indicator 
and HARQ index (\textsf{harq}) inside the control channel, 
tracking the rate of recent re\hyp{}transmissions for each cell. 
LTE encodes each control message using a 1/3 rate convolutional code, then appends a 16-bit CRC after the payload. 

\subsubsection{LTE Control Channel Decoding}

The control channel consists of \textit{control channel elements} (CCEs), 
each of which is a group of 72 coded bits, as shown in Figure~\ref{fig:cce_list}.
LTE transmits one control message using $L$ consecutive CCEs, where $L=1,2,4,8$ 
is the \textit{aggregation level}. 
To simplify the decoding process, a control message with 
aggregation level $L$ must only start at a 
CCE index that is
a multiple of $L$, as shown in Figure~\ref{fig:cce_list}. 
To reduce computational overhead, LTE assigns a 
UE-specific \textit{search space} for a UE, which is a group
of consecutive CCEs
with starting index given by a hash of
the \textsf{C-RNTI}, subframe index, and aggregation level
\cite{LTE_UMTS}.
Each coded control message is either punctured 
or repeated to fit into $L$ CCEs.

\begin{figure}[htb]
    \centering
    \includegraphics[width=0.99\linewidth]{fig/CCE_list.pdf}
    \caption{LTE groups 72 coded bits into a control channel element (CCE). 
    One control message occupies one or multiple consecutive CCEs, depending
    on the aggregation level $L$.}
    \label{fig:cce_list}
\end{figure}

A UE attempts to decode a control message at every 
possible control message position at a given aggregation level.
For example, searching at CCE index 14, as shown 
in Figure~\ref{fig:cce_list}, the UE takes 
the coded bits inside CCEs 14 and 15, undoes the bit 
puncturing or repeating according to each control format, and 
decodes the possible control message therein using a
convolutional decoder. 
The decoded message consists of 
the message payload and a 16-bit $CRC$, as shown in 
Figure~\ref{fig:rnti}. The UE calculates another $CRC^{\prime}$ 
using the decoded message payload and exclusive-ors the 
appended $CRC$ with $CRC^{\prime}$. 
The resulting 16-bit sequence is the physical layer
ID (\textsf{C-RNTI}) of the intended receiver of this message. 
The UE then searches for a message that has its own
C-RNTI, and only decodes control messages at those positions.

% \subsection{Decoding process of a standard UE} \label{s:ue_decode}
% \textcolor{blue}{The UE's physical layer ID \textit{C-RNTI} (a 16-bit integer) is a key parameter for UE to decode the control channel. First of all, \textit{C-RNTI} is used by the LTE to indicate the intended receiver of each control message inside the control channel. Second, the \textit{C-RNTI} helps the UE to significantly reduce the decoding computation overhead. }
\begin{figure}[htb]
    \centering
    \includegraphics[width=\linewidth]{fig/decoder.pdf}
    \caption{Testing control message format type using the computed
    check-sum and the user identifier.}
    \label{fig:rnti}
    \label{fig:rntia}
\end{figure}

The key challenge here is that \systemname{} does not know the 
physical layer ID \textsf{C-RNTI} of any UE. 
Without \textsf{C-RNTI}, \systemname{} is not able to reduce 
the search space using the above UE\hyp{}specific search space. 
Searching all control message positions would generate
thousands of messages, \eg, the control channel 
of a 20~MHz cell could generate 1,570 messages.  
%\systemname{} cannot identify the real control message that the cell 
%tower transmits without the ID of the receiver. 
In the following, we describe how \systemname{} reduces the search space and how it performs joint
decoding and identification of control messages.
\begin{figure*}[!t]
    \begin{subfigure}[b]{0.24\linewidth}
    \centering
    \includegraphics[width=0.98\linewidth]{fig/tree_a.pdf}
    \caption{Aggregation level.}
    \label{fig:tree_a}
    \end{subfigure}
    \begin{subfigure}[b]{0.27\linewidth}
    \centering
    \includegraphics[width=0.98\linewidth]{fig/tree_b.pdf}
    \caption{Pruning according to LLR.}
    \label{fig:tree_b}
    \end{subfigure}
    \begin{subfigure}[b]{0.20\linewidth}
    \centering
    \includegraphics[width=0.97\linewidth]{fig/tree_c.pdf}
    \caption{Rate matching.}
    \label{fig:tree_c}
    \end{subfigure}
    \begin{subfigure}[b]{0.27\linewidth}
    \centering
    \includegraphics[width=0.98\linewidth]{fig/tree_d.pdf}
    \caption{Pruning after decoding.}
    \label{fig:tree_d}
    \end{subfigure}
\caption{Packet loss and retransmission interacts with
LTE's H-ARQ design to cause a packet arrival delay 
followed by a burst of packets.}
\label{fig:tb_delay_combined}
\end{figure*}


\subsubsection{Search Space Reduction} 

% Without \textit{C-RNTI}, \systemname{} is not able to identify whether one decoding attempt is successful or not.  Therefore, \systemnames{} goal is to decode every control message in the control channel, to get a full picture about the resource allocation for every subframe. \systemname{}, however, does not know the physical layer ID \textit{C-RNTI} of any UE. Therefore, \systemname{} is not able to reduce the search space as the standard UE does. Furthermore, \systemname{} cannot tell whether the decoding is successful after conducting one decoding attempt. 

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.8\linewidth]{fig/CCE_main.pdf}
    \caption{The per-bit log-likelihood-ratio (LLR) values indicate the confidence of each coded bit inside one CCE. Consecutive non-empty CCEs form a \textit{CCE group}.}
    \label{fig:cce_main}
\end{figure}

% \subsubsection{\systemnames{} Decoding Process} 
% In this section, we describe the control channel decoding process of \systemname{}. \systemname{} reduces search space via identifying the empty CCEs. 


To reduce the search space, \systemname{} identifies all the empty CCEs inside the control channel. Specifically, we inspect the confidence values, \ie, the log-likelihood ratios (LLRs), for each bit inside a CCE, as shown in Figure~\ref{fig:cce_main}. When the CCE is empty, no bits are actually transmitted, so the confidence values of the bits inside such a CCE are close to zero. We, therefore, identify a CCE as empty if the average LLR of the demodulated (coded) bits inside it is below a hard threshold (0.85 in our implementation), which is selected to balance the size of the search space and true positive. Specifically, with a threshold of zero, no empty CCEs are detected and the search space is maximized. Increasing the threshold leads to more empty CCE being identified and smaller search space, which, however, increases the possibility that an occupied CCE is missed. We search for the highest threshold (smallest search space) that can constantly achieve a true positive rate of 98\% over 100 traces.

From the search space hashing process, we see that multiple possible combinations of 
control messages may be packed into the positions our LLR indicator indicates, which
we term \textit{CCE groups}.
For example, in Figure~\ref{fig:cce_main}, the $0^{\mathrm{th}}$ and $1^{\mathrm{st}}$ CCEs 
could be used to deliver one $L=2$ control message or two separate $L=1$ control 
messages, but the $3^{\mathrm{rd}}$ and $4^{\mathrm{th}}$ CCEs must be used to 
deliver two separate messages, as an $L=2$ message 
cannot start at index three. From the CCE groups, 
we construct a \textit{control message location list} that lists all possible positions of the control message.
\systemname{} performs decoding attempts for possible control 
message positions inside the control message location 
list.

\subsubsection{Message validation via temporal UE tracking}
\label{s:dci_val}
Each decoding attempt generates 10 candidates decoded control messages 
(one for each possible message format), so
our goal is to jointly verify the candidate message and 
extract the \textsf{C-RNTI} of the intended receiver. 
Our key observation is that \textsf{C-RNTIs} that reappear within a short 
period of time (16~$ms$ in our implementation) are likely 
real, as \textsf{C-RNTIs} calculated using a wrong format are random
and evenly distributed. The possibility of re-hitting the same 
\textsf{C-RNTI} generated using wrong formats can be calculated according to the birthday problem~\cite{Birthday},
which is extremely small, as the space of possible \textsf{C-RNTIs} 
is $2^{16}$ in size. 
For example, the possibility that
two \textsf{C-RNTIs} reappear within 1,000 messages are $1\times10^{-4}$.
% \todo{why??? cite B-Day Paradox}

We design a \textit{UE Tracker} to first store the derived 
\textsf{C-RNTIs} together with the corresponding control messages and track the ID of real UE. 
The tracker uses a ring buffer to buffer the messages from 16 recent subframes and
maintains a \textit{temporary ID list} that stores the count of appearances of 
each \textsf{C-RNTI} in the ring buffer, 
as shown in Figure~\ref{fig:ue_tracker}.
If a \textsf{C-RNTI} count is larger than 
two, we identify it as the ID of a real UE and move it to the 
\textit{detected UE} list.
The tracker searches the ring buffer for messages associated with
\textsf{C-RNTIs} in the UE list, which are identified as 
valid control messages. 
We record the \textit{last active time} of each \textsf{C-RNTI} 
(the index of the most recent subframe that this \textsf{C-RNTI} is observed). 
A \textsf{C-RNTI} that is inactive for 10 seconds is removed from the list.

To reduce the number of buffered messages, we filter out messages with 
a large 
number of coded bit errors by re-encoding each decoded control message
into coded bits, then comparing the result with the original coded bits 
inside the received CCEs to calculate the ratio of 
bits that are erroneous. We drop messages with more than 25\% code bits flipped,
which is a very high threshold that filters out extremely noisy messages and misses almost no true positive messages, while allowing
false positives through, which however are not identified as the ID of real UEs by our UE Tracker.

% are later filtered by the UE tracker, which we describe next.
\begin{figure}[tbh]
    \centering
    \includegraphics[width=0.98\linewidth]{fig/UE_tracker.pdf}
    \caption{The \systemname{} \textit{UE Tracker}. 
    \systemname{} buffers recent decoding results, 
    maintaining a list tracking
    each \textsf{C-RNTI's} recent prevalence.} 
    \label{fig:ue_tracker}
\end{figure}

To accelerate the decoding process, we identify \textit{active UEs} by 
counting the number of decoded control messages in the past 
second and decode their UE-specific search space with high priority. 
We expect active UEs' communication will continue in the near future, 
so that it is highly possible to find control messages inside the 
UE-specific search space of the active UEs. 
We sort \textsf{C-RNTIs} in decreasing message count and
immediately output a message if the \textsf{C-RNTI} matches the
ID of the active UE and otherwise buffer it.
We stop decoding one subframe if the total allocated PRB inside all 
identified control messages equal to the PRB of the cell tower.


\parahead{UE tracking with carrier aggregation} 
When carrier aggregation is active, each aggregated cell tower transmits its 
own control messages to the same UE through its respective control channel.
A UE has only one physical layer ID \textsf{C-RNTI}, and so
the \textsf{C-RNTI} of a UE being served by carrier aggregation 
appears in the control messages transmitted by all aggregated cells. 
The master maintains a copy of the detected UE list of all slaves, 
which are updated every 10~$ms$ by slaves. 
The master then extracts the intersected \textsf{C-RNTI}s across the UE lists of all slaves, 
which are identified as the ID of UEs with carrier aggregation enabled.
According to the lists the ID appears in, the master derives the UE's aggregated cells. 
What's more, the master identifies the primary and secondary cells of the UE according to the time the ID appears in each list.
Carrier aggregation is triggered only when the LTE network has a large volume of data for the UE, as shown in Figure~\ref{fig:CA_RATE_all}. 
We, therefore, filter out any detected UEs whose traffic load 
falls below a rate of 3 Mbit/s, determined experimentally
based on our traffic traces as well as an inspection of when carrier aggregation 
is triggered (or not).


\subsection{Data Fusion}
\label{s:fusion}

From Figure~\ref{fig:system}, we see that the master PC decodes the control 
messages by itself, and at the same time receives control messages decoded 
by slaves, so the master needs to synchronize control messages from different
sources. The subframe index provides a timestamp for each control message,
and since all LTE cell towers are tightly time synchronized these 
subframe index timestamps 
provide a consistent ordering of messages. 

The master PC also receives a packet reception log from the UE. 
To infer packet status inside the LTE network in real time, the 
master PC must synchronize and align the cross layer information,
\ie, the steam of LTE physical layer control message and the 
UE transport layer packet log.  This requires two tasks: 
first, we need to associate the \textsf{C-RNTI} with the \systemname{} 
UE. The \textsf{C-RNTI}, is assigned by the 
LTE cell tower and delivered to the UE through an encrypted data channel. 
LTE chips on the commercial mobile phones do not expose the 
\textsf{C-RNTI} to the OS since it is only used in 
the LTE physical layer. Without the \textsf{C-RNTI} of the \systemname{}
UE, we are not able to directly identify which control message is
transmitted to that specific UE. Second, we need to remove the time 
shift between the timestamp of the control message and the timestamp
of the packet arrival. If we knew the \textsf{C-RNTI} of the UE under
test, we would know how many bits are sent to the UE in each subframe 
according to the control message. We, however, are not able to link 
the bits sent over each subframe with the packets received by the UE,
without removing the time shifts between timestamps of control message 
and packet log.

We leverage the packet arrival pattern caused by 
LTE retransmissions, to associate the \textsf{C-RNTI} with the UE 
under test and eliminate the shift between timestamps. 
Specifically, we transmit UDP traffic with data rate 10~Mbit/s for 
5 seconds, from a server that is at the edge of the network to 
the UE under test. We record the packet log at the UE and 
decode the control channel. From the decoded control message, 
we can identify the starting and ending subframe for each 
retransmission, as shown in Figure~\ref{fig:tb_err_burst}. 
From the packet log, we can also detect a retransmission based on 
the eight millisecond delay and the packet burst. We 
shift the timestamp of the packet log to match the locations of 
the retransmissions inside the packet log and the control 
message with the \textsf{C-RNTI}. The control message with the 
highest amount of matching retransmissions is identified 
as the message of the UE under test.  
By doing so, we synchronize the packet log with control message to 
an eight millisecond precision. 
From the decoded control messages, we know the subframe in which the 
retransmission finishes. Therefore, we align the packet log with the 
control message by shifting the packet arrival burst into the corresponding subframe. 
If there are multiple close\hyp{}by retransmissions, we can differentiate them by checking 
the length of the burst, thus
refining our synchronization to millisecond precision. 






==> E2E.tex <==
\section{End-to-End Congestion Control}
\label{s:e2e}
\label{s:motivation}

This section sketches a preliminary design of an improved end-to-end 
congestion control algorithm that \systemname{} makes possible for 
the first time, further motivating our approach.

When congestion is caused by packet queuing in the wired network, typically many
connections experience it at the same time, competing for bandwidth at the bottleneck link.  
On the other hand, when congestion is caused by lack of capacity at the wireless cell, 
each user has its own buffer and channel resources allocated to it.
In both cases, the goal of a congestion control algorithm is to adapt the sender's rate 
to the available end\hyp{}to\hyp{}end capacity, but the means of estimating this 
capacity should differ based on whether congestion is at a wired or wireless link, 
for the following reasons.
In the former case, relying on end\hyp{}to\hyp{}end signals has been shown to work 
well \cite{CUBIC,BBR,XCP}.  In the latter case, the congestion may vary at timescales
much smaller than end\hyp{}to\hyp{}end signals can capture, and so this congestion 
must be measured using the new techniques \systemname{} introduces below.  
Furthermore, in the latter case, since each user has its own buffer, each user 
has little to no impact on end\hyp{}to\hyp{}end signals such as latency, and 
so physical\hyp{}layer techniques should be leveraged.

\paragraph{New challenge:\ Carrier aggregation.}
Therefore a wireless\hyp{}aware congestion control algorithm should first 
ascertain the extent to which the base station is the bottleneck, at highly granular time scales. 
While control messages expose LTE resource allocation data, allowing the 
measurement of a single cell's utilization to this end \cite{OWL, LTEye},
carrier aggregation may further cause one LTE link to in fact traverse multiple
cell towers, as shown in Figure~\ref{fig:CA_main}. In this case, the (cellular) bottleneck
depends not solely on a single tower, but instead on all cell towers the connection traverses.


The aggregate wireless link capacity depends broadly on at least 
four parameters:\ carrier aggregation, 
\textit{modulation and coding rate} (MCS), the number of MIMO
spatial streams, the \textit{available} frequency bandwidth 
(\ie, the PRBs allocated for that user plus the idle PRBs in the cell),
and finally the packet delivery rate.  The former four parameters
can vary every subframe, and so our design (\S\ref{s:design}) 
tracks them at this granularity.  Furthermore, the latter parameter,
specifically the presence of 
link\hyp{}layer retransmissions, reshapes the packet delivery pattern 
at the transport\hyp{}layer socket, thus fundamentally 
affecting the end\hyp{}to\hyp{}end inter-packet-arrival time 
and round trip time measurements that in prior works use in 
their end\hyp{}to\hyp{}end capacity estimates, as we now explain. 

\begin{figure}[!t]
    \begin{subfigure}[b]{\linewidth}
    \centering
    \includegraphics[width=0.98\linewidth]{fig/tool_reTx.pdf}
    \caption{TB loss and reception; packet delivery at socket.}
    \label{fig:tb_err_burst}
    \end{subfigure}
    \vspace*{0.25ex}
    
    \begin{subfigure}[b]{\linewidth}
    \centering
    \includegraphics[width=0.98\linewidth]{fig/TB_reTx_delay.pdf}
    \caption{TB reception (bits) and one\hyp{}way delay.}
    \label{fig:tb_reTx_delay}
    \end{subfigure}
\caption{Packet loss and retransmission interacts with
LTE's H-ARQ design to cause a packet arrival delay 
followed by a burst of packets.}
\label{fig:tb_delay_combined}
\end{figure}

Figure~\ref{fig:tb_err_burst} 
shows an example of TB failure and retransmission.
Here the UE fails to decode a TB in 
the first subframe that contains a transport layer packet with sequence 
number~1. Eight milliseconds after the original transmission, the LTE cell tower 
retransmits the lost TB, in Subframe~9.  However, as we have explained above, the base station continues transmitting data to the UE 
in the subframes between the original transmission and the retransmission 
(Figure~\ref{fig:harq_flow}).  Assuming many TBs sent 
over subframes two to eight are decoded correctly, the UE receives 
packets with sequence number two to ten before the reception of a packet 
with sequence number one, causing many out-of-order packet receptions.
To prevent out-of-order packet reception from happening at higher layer, 
the LTE link layer ensures in-order TB delivery, numbering each TB, 
checking its sequence number, and buffering any and all out-of-order TBs
in a \textit{reorder buffer} until the retransmission recovers the missing TB(s). 
The link layer then extracts packets from the TBs and delivers them to the 
receiving socket, resulting in a burst of packets received at that layer. 
Furthermore, Figure~\ref{fig:tb_reTx_delay} shows that the
burst also reshapes the inter-packet-arrival time and round-trip-time that most existing congestion
control algorithms rely on as a control signal 
\cite{Sprout,Copa,BBR,CUBIC,Verus}. 
The packets inside the burst in fact arrive at the UE uniformly, but are
instead reported together, creating a large interval between the 
burst and the packets received before the burst. 
The congestion algorithms should therefore compensate 
for this effect, to obtain meaningful estimates of the 
end\hyp{}to\hyp{}end channel capacity.

==> Intro_atc.tex <==
\section{Introduction}
\label{s:intro}
Cellular networks accounted for 72\% of global traffic in the past few years, 
with this trend expected to continue through 2022~\cite{CiscoReport}.  
Motivated by this, the research community is devoting significant 
effort to improve the congestion control design of end\hyp{}to\hyp{}end transport connections, 
so key applications such as video conferencing,
video delivery~\cite{CellurVideo,MuVi,Pensieve,Sprout,Salsify}, and bulk data transfer~\cite{PCC-v,PCC,Copa,CUBIC,BBR,Verus}, 
can work seamlessly with the wireless network, 
whose link capacity varies significantly within a very short period of time. 

An end\hyp{}to\hyp{}end connection may exist in three different states at the bottleneck link: \textit{under-utilization} where the offered load is below the network capacity and no queues form; 
\textit{over-utilization} where the offered load is greater than the capacity and queues form; 
and \textit{saturation} where buffers are filled and packet loss occurs, as shown in Figure~\ref{fig:tcp_state}. 
Loss-based congestion control algorithms alternate between saturation and under-utilization by first increasing the offered load to fill the buffer and backoff quickly to drain the queue, 
and has been the dominant solution for more than 10 years. 
BBR~\cite{BBR}, however, proves that end\hyp{}to\hyp{}end connections can work reliably at the ``sweet spot'' between under-utilization and over-utilization, 
without forming queues, simultaneously achieving high throughput and low delay.
\begin{figure}[tb]
    \centering
    \begin{subfigure}[b]{0.99\linewidth}
        \centering
        \includegraphics[width=\textwidth]{fig/intro_3app_a.pdf}
        \caption{Congestion control matches sending rate to channel capacity.}
        \label{fig:3app_transport}
    \end{subfigure}
    
    \begin{subfigure}[b]{0.99\linewidth}
        \centering
        \includegraphics[width=\textwidth]{fig/intro_3app_b.pdf}
        \caption{Server adapts the streaming video quality to channel capacity.}
        \label{fig:3app_vod}
    \end{subfigure}
    
    \begin{subfigure}[b]{0.99\linewidth}
        \centering
        \includegraphics[width=\textwidth]{fig/intro_3app_c.pdf}
        \caption{Mobile user adjusts video encoding quality to channel quality.}
        \label{fig:3app_conference}
    \end{subfigure}
    
   \caption{Channel capacity is required by 
    the congestion control algorithms of the transport layer protocol (\textbf{a});
   video on demand (\textbf{b});
    and video telephony (\textbf{c}).  
   }
    \label{fig:CA_example}
\end{figure}

%\begin{figure}[tbh]
%    \centering
%    \includegraphics[width=0.98\linewidth]{fig/TCP_state.pdf}
%    \caption{The three possible congestion states of the bottleneck link of an end\hyp{}to\hyp{}end connection.} 
%    \label{fig:tcp_state}
%    % \vspace{-0.5cm}
%\end{figure}

To work at the sweet spot, congestion control algorithms like BBR must estimate a key parameter---the \textit{bottleneck capacity}---and set the sending offered load to the estimated capacity. 
The bottleneck capacity of an end\hyp{}to\hyp{}end connection built atop a wireless cellular networks exhibits significant variations even over short time durations. 
This is because the wireless last hop is, most of the time, the bottleneck of the end\hyp{}to\hyp{}end connection~\cite{CQIC,Verus,MaoInDepth,LteMeasureHighWay,highway}, 
whose capacity varies at millisecond level time scales for three main reasons:
\begin{enumerate}
  \item Wireless channel quality between cell tower and the user varies across time and space. The highest modulation and coding rate the link can support changes accordingly.
  
  \item The available bandwidth for one specific mobile user (including the allocated bandwidth for the UE and idle bandwidth of the cell), varies. Within one cell, many users share available bandwidth, so competition between users affects this resource allocation. 
  
%   \item The effective channel bandwidth used for data transmission varies because of data bit errors. From our observation, LTE cell towers spend a large portion (8\% to 14\%) of their bandwidth retransmitting previously\hyp{}errored data.

    \item Both the LTE-Advanced~\cite{LTE-Rel-10} and the 5G networks~\cite{5G} use a technique called \textit{carrier aggregation (CA)} in which two or more frequency ranges (called \textit{component carriers}) are aggregated and assigned to one user to support higher per\hyp{}user data rates. Because of carrier aggregation, one end\hyp{}to\hyp{}end connection is not only affected by the dynamics from one cell but from all of its aggregated cells.
\end{enumerate}
% What further complicates the situation is that, recent LTE-Advanced (3GPP Release 10 and onward) uses a technique called \textit{carrier aggregation} in which two or more frequency ranges (called \textit{component carriers}) are aggregated and assigned to one user to support higher per\hyp{}user data rates. An example is shown in Figure~\ref{fig:CA_main}: the UE associates with its primary cell which operates over a 10~MHz channel at 2.1~GHz. A secondary serving cell operating over a 20~MHz channel at 800~MHz can be aggregated to achieve 30~MHz bandwidth. Because of carrier aggregation, one TCP link is not only affected by the dynamics from one cell but from all of its aggregated cells. 
% \begin{figure}[th] 
%   \centering
%   \includegraphics[width=0.92\linewidth]{fig/CA_main.pdf}
%   \caption{\textit{Carrier aggregation:}\ Multiple towers operating at different frequencies and bandwidths
%   serve a single user.} 
%   \label{fig:CA_main}
% \end{figure}


The rapidly varying cellular network dynamics put congestion control design in a dilemma---on one hand, the congestion control algorithm should estimate the bottleneck capacity with fine granularity and adjust its sending rate as fast as possible to cope with the variations of the cellular network; on the other hand, it should not over-react to random network glitches introduced by short-lived data flows.
Without knowing the internal state of wireless cellular link, BBR and BBR-like algorithms such as Sprout\cite{Sprout}, Verus~\cite{Verus}, PCC~\cite{PCC,PCC-v} and COPA~\cite{Copa} treat the wireless cellular network as a black box, relying on end-to-end packet statistics to estimate the channel capacity, resulting in either under-utilization of the network capacity or excessive delay (\S\ref{s:congestion}). 
% The goal of designing a congestion control algorithm that achieves simultaneously high throughput and low latency.
% \begin{figure}[tb]
%     \centering
%     \includegraphics[width=0.7\linewidth]{fig/ATC_thput.pdf}
%     \caption{Throughput and packet delay of seven congestion control algorithms over a commercial cellular network. 
%     We test 20 links and each algorithm over a link for 20 seconds. } 
%     \label{fig:cca_test}
%     % \vspace{-0.5cm}
% \end{figure}

\parabreak The observation we make in this  paper is that, the cell tower broadcasts
all the wireless parameters that affect the bottleneck capacity, including the \textit{modulation and coding rate} (MCS), 
the number of MIMO spatial streams, the allocated frequency bandwidth, the number of retransmissions, and the aggregated cell towers, to the mobile users via a physical control channel. 
By carefully decoding this physical control channel, we can expose the internal state of the wireless cellular network to transport layer and applications at the endpoints,
opening new possibilities for better congestion control design for cellular networks.
% Researchers have begun to tackle the challenge of understanding LTE's operation at fine time scales. 
Passive cellular sniffers such as LTEye~\cite{LTEye} and OWL~\cite{OWL} already decode the control channel to infer some of the above wireless attributes, 
but cannot work with the most cutting edge cellular that uses techniques such as carrier aggregation, and thus is not able to track the abrupt capacity change the carrier aggregation causes, as the example in Figure~\ref{fig:CA_example} shows.
MobileInsight~\cite{MobileInsight} can only analyze the radio resource allocation of a single UE rather than cell-wide information, which is however, mandatory in order to
estimate the capacity available to the mobile users.


This paper presents the design and implementation of \textit{\systemname{}},
a tool that exposes the fine-grained information applications and transport protocols require 
for superior performance. 
\systemname{} simultaneously decodes the physical layer control channels of
multiple cell towers using off-the-shelf software-defined radios, extracting highly
granular, per\hyp{}user link and physical layer transmission status information for 
all users.  By combining these data across users within one cell, and fusing data across cells, \systemname{} observes and accounts for the effects of carrier aggregation, estimating network load more accurately than previous cellular monitors.
By reconciling control messages from the cellular physical layer with the packet arrival time series from the UE's transport layer, we accurately monitor the downlink delivery process of every packet the UE receives across layers and down to the PHY, enabling the better functionality of congestion control algorithms, which heretofore lacked insight into the PHY.

\begin{figure}[tb]
    \centering
    \begin{subfigure}[b]{0.49\linewidth}
        \centering
        \includegraphics[width=\textwidth]{fig/ATC_CA_example_a.pdf}
        \caption{The allocated bandwidth.}
        \label{fig:CA_allocatedB}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.49\linewidth}
        \centering
        \includegraphics[width=\textwidth]{fig/ATC_CA_example_b.pdf}
        \caption{The packet delay.}
        \label{fig:CA_oneway}
    \end{subfigure}
    \caption{An example of CA triggering. The offered load of the server (25~Mbit/s) exceeds the 
    capacity the 5~MHz cell, resulting in packet queuing. Cellular network aggregates a 20~MHz cell to boost the maximum capacity of such a user.  }
    \label{fig:CA_example}
    \vspace{-0.5cm}
\end{figure}
We have implemented \systemname{} with multiple USRP 
software-defined-radios, host PC, and a mobile phone in a design that synchronizes 
and fuses information from these sources.  
Our performance evaluation 
presents end\hyp{}to\hyp{}end measurements in a commercial cellular network
to validate the accuracy and measurement resolution
of \systemname{} in both static and mobile user scenarios.
\systemnames{} control channel decoder
achieves a reduction in missed control messages to 0.8\% (a 82\% reduction over OWL). 
\systemname{} also reduces the rate of false positives (detection of nonexistent control messages) by 92\% compared to OWL.
Results show that wireless capacity varies significantly with mobility, transmission errors, competing traffic within each cell and the
number of aggregated cells when carrier aggregation is triggered (\S\ref{s:eval_capEst}). \systemname{}
tracks the resulting capacity variations with collected cross-layer information
at millisecond granularity, enabling more effective congestion control algorithms.

We also make new experimental observations on cellular wireless physical\hyp{} and 
link\hyp{}layer operations.
% Firstly, we observe that as offered load increases, the  size of a data frame at the physical layer increases, thus increasing the probability of a frame loss, even when modulation and coding rate stay constant. We explain this phenomenon by comparison with a theoretical prediction of the same effect. Furthermore, indoors when the UE is mobile, the bit rate adaptation algorithm cannot track the resulting small scale multipath fading fast enough, resulting in consistently high levels of packet loss that are independent of data frame size. 
Firstly, we find that some cell towers only function as a secondary cells to deliver carrier\hyp{}aggregated downlink traffic (\S\ref{s:eval_capEst}). 
Without competition from primary users, such a cell ensures a stable capacity boost for UEs, motivating a congestion control that can exploit such an opportunity. 
Secondly, we observe that with carrier aggregation enabled,the cellular network saturates the primary cell (in our \S\ref{s:eval_CA_cells} example the spectrum efficiency is 2.4~Mbit/s/Hz) before the secondary
(2.6~Mbit/s/Hz) and tertiary cells(8.4~Mbit/s/Hz), resulting in inefficient bandwidth usage. 
Lastly, we observe cross-cell traffic correlation (\S\ref{s:eval_compete}), the effect of competing traffic propagating to other cells via carrier aggregation.

==> MacRetran.tex <==
\section{Evaluation}
In this section, we evaluate the performance of \systemname\ in measuring the LTE MAC and PHY layer operations. We also evaluate the 
\begin{figure*}[!t]
    \centering
    \begin{minipage}[b]{0.32\linewidth}
        \centering
        \includegraphics[width=\textwidth]{fig/reTx_tb_ratio.pdf}
        \caption{The ratio of retransmission in the total data that sent from the cell tower to the UE.}
        \label{fig:reTx_ratio}
    \end{minipage}
    \hfill
    \begin{minipage}[b]{0.32\linewidth}
        \centering
        \includegraphics[width=\textwidth]{fig/tbs_cdf.pdf}
        \caption{The ratio of subframes transmitted with one spatial stream (maximum two streams allowed).}
        \label{fig:tbs_cdf}
    \end{minipage}
    \hfill
    \begin{minipage}[b]{0.32\linewidth}
        \centering
        \includegraphics[width=\textwidth]{fig/FER_size.pdf}
        \caption{Packet loss rate when remote server sending UDP packets with different sending speed.}
        \label{fig:FER_size}
    \end{minipage}
    \hfill
    
    % \vspace{-10pt}
\end{figure*}

\subsection{LTE errors and retransmissions}
\systemname is able to identify the every retransmitted transport block. In this section, we investigate the frequency of retransmissions in commercial LTE network and the impact to LTE packet transmissions. 

\parahead{Experiment setup} We set up a remote server on Amazon AWS cloud as the sender. We use a Samsung Glaxsy S8 with unlimited data plan as the receiver. We build a UDP connection between the remote server and the phone. In our static experiment, we place the mobile phone at one location and let the remote server send date through the UDP link at one speed for 10 seconds. We vary the speed of the remote server from 10~Mbit/s to 55~Mbit/s in one location. We move the phone to 10 locations in a building where the signal strength of the cell tower varies from -85~dBm to -113~dBm. The phone is connected with the same cell tower during the experiment.
We decode the control channel and extract the new-data indicator, from which we count how many transport blocks have retransmissions. We calculate the ratio of transport blocks to the total number of transmitted transport blocks and plot the results in Figure~\ref{fig:reTx_ratio}.  



% \begin{figure*}
%     \begin{minipage}[t]{0.32\textwidth}
%       \begin{subfigure}[t]{0.98\linewidth}
%          \centering
%          \includegraphics[width=0.98\linewidth]{fig/CA_rate0_a.pdf}
%           \caption{Oneway delay at UE.}
%           \label{fig:ue_rx_rate}
%       \end{subfigure}\hfill
      
%       \begin{subfigure}[t]{0.98\linewidth}
%          \centering
%          \includegraphics[width=0.98\linewidth]{fig/CA_rate0_b.pdf}
%           \caption{PRB allocation of cell one.}
%           \label{fig:ue_rx_data}
%       \end{subfigure}\hfill
      
%       \begin{subfigure}[t]{0.98\linewidth}
%          \centering
%          \includegraphics[width=0.98\linewidth]{fig/CA_rate0_c.pdf}
%           \caption{PRB allocation of cell four.}
%           \label{fig:ue_rx_data}
%       \end{subfigure}\hfill
      
%       \begin{subfigure}[t]{0.98\linewidth}
%          \centering
%          \includegraphics[width=0.98\linewidth]{fig/CA_rate0_d.pdf}
%           \caption{PRB allocation of cell five.}
%           \label{fig:ue_rx_data}
%       \end{subfigure}\hfill
%       \caption{Cap1.}
%       \label{fig:ue_DataRate}
%     \end{minipage}\hfill
%     \begin{minipage}[t]{0.33\textwidth}
%         \begin{subfigure}[t]{0.98\linewidth}
%          \centering
%          \includegraphics[width=0.98\linewidth]{fig/CA_rate0_a.pdf}
%           \caption{Oneway delay at UE.}
%           \label{fig:ue_rx_rate}
%       \end{subfigure}\hfill
      
%       \begin{subfigure}[t]{0.98\linewidth}
%          \centering
%          \includegraphics[width=0.98\linewidth]{fig/CA_rate0_b.pdf}
%           \caption{PRB allocation of cell one.}
%           \label{fig:ue_rx_data}
%       \end{subfigure}\hfill
      
%       \begin{subfigure}[t]{0.98\linewidth}
%          \centering
%          \includegraphics[width=0.98\linewidth]{fig/CA_rate0_c.pdf}
%           \caption{PRB allocation of cell four.}
%           \label{fig:ue_rx_data}
%       \end{subfigure}\hfill
      
%       \begin{subfigure}[t]{0.98\linewidth}
%          \centering
%          \includegraphics[width=0.98\linewidth]{fig/CA_rate0_d.pdf}
%           \caption{PRB allocation of cell five.}
%           \label{fig:ue_rx_data}
%       \end{subfigure}\hfill
%       \caption{CAP2.}
%       \label{fig:ue_DataRate}
%     \end{minipage}\hfill
%     \begin{minipage}[t]{0.33\textwidth}
%         \begin{subfigure}[t]{0.98\linewidth}
%          \centering
%          \includegraphics[width=0.98\linewidth]{fig/CA_rate0_a.pdf}
%           \caption{Oneway delay at UE.}
%           \label{fig:ue_rx_rate}
%       \end{subfigure}\hfill
      
%       \begin{subfigure}[t]{0.98\linewidth}
%          \centering
%          \includegraphics[width=0.98\linewidth]{fig/CA_rate0_b.pdf}
%           \caption{PRB allocation of cell one.}
%           \label{fig:ue_rx_data}
%       \end{subfigure}\hfill
      
%       \begin{subfigure}[t]{0.98\linewidth}
%          \centering
%          \includegraphics[width=0.98\linewidth]{fig/CA_rate0_c.pdf}
%           \caption{PRB allocation of cell four.}
%           \label{fig:ue_rx_data}
%       \end{subfigure}\hfill
      
%       \begin{subfigure}[t]{0.98\linewidth}
%          \centering
%          \includegraphics[width=0.98\linewidth]{fig/CA_rate0_d.pdf}
%           \caption{PRB allocation of cell five.}
%           \label{fig:ue_rx_data}
%       \end{subfigure}\hfill
%       \caption{CAP3.}
%       \label{fig:ue_DataRate}
%     \end{minipage}\hfill
% \end{figure*}



\begin{figure}[!t]
    \centering
    \includegraphics[width=0.98\linewidth]{fig/cell_rate_inc.pdf}
    \caption{The difference between two consecutively received packets..}
    \label{fig:tbs_cdf}
\end{figure}

\begin{figure*}[!t]
    \centering
    \begin{subfigure}[b]{0.245\linewidth}
        \centering
        \includegraphics[width=\textwidth]{fig/mcs_cdf_a.pdf}
        \caption{RSRP -76dBm, load 25Mbps.}
        \label{fig:tbs_cdf}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.245\linewidth}
        \centering
        \includegraphics[width=\textwidth]{fig/mcs_cdf_b.pdf}
        \caption{RSRP -76dBm, load 40Mbps.}
        \label{fig:tbs_cdf}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.245\linewidth}
        \centering
        \includegraphics[width=\textwidth]{fig/mcs_cdf_c.pdf}
        \caption{RSRP -95dBm, load 40Mbps.}
        \label{fig:tbs_cdf}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.245\linewidth}
        \centering
        \includegraphics[width=\textwidth]{fig/mcs_cdf_d.pdf}
        \caption{RSRP -115dBm, load 40Mbps.}
        \label{fig:tbs_cdf}
    \end{subfigure}
    \hfill
    % \vspace{-10pt}
\end{figure*}

\begin{figure}[!t]
    \centering
    \begin{subfigure}[b]{0.98\linewidth}
        \centering
        \includegraphics[width=\textwidth]{fig/reTx_len_dB.pdf}
        \caption{Offered load 40Mbps.}
        \label{fig:tbs_cdf}
    \end{subfigure}
    \hfill
    
    \begin{subfigure}[b]{0.98\linewidth}
        \centering
        \includegraphics[width=\textwidth]{fig/reTx_len_Mbps.pdf}
        \caption{Cell RSRP -95dBm.}
        \label{fig:tbs_cdf}
    \end{subfigure}
    \hfill
   
\end{figure}

% \begin{figure}[!t]
%     \centering
%     \begin{subfigure}[b]{0.98\linewidth}
%         \centering
%         \includegraphics[width=\textwidth]{fig/tbs_cdf_subframe.pdf}
%         \caption{Number of bits transmitted within each subframe (cell RSRP -87dBm).}
%         \label{fig:tbs_cdf}
%     \end{subfigure}
%     \hfill
    
%     \begin{subfigure}[b]{0.98\linewidth}
%         \centering
%         \includegraphics[width=\textwidth]{fig/tbs_cdf_stream.pdf}
%         \caption{Number of bits transmitted through one spatial stream (RSRP -87dBm).}
%         \label{fig:tbs_cdf}
%     \end{subfigure}
%     \hfill
   
% \end{figure}


% \begin{figure}[!t]
%     \centering
%     \begin{subfigure}[b]{0.49\linewidth}
%         \centering
%         \includegraphics[width=\textwidth]{fig/prb_cdf.pdf}
%         \caption{Allocated PRBs.}
%         \label{fig:tbs_cdf}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.49\linewidth}
%         \centering
%         \includegraphics[width=\textwidth]{fig/prb_efficy.pdf}
%         \caption{Spectrum efficiency.}
%         \label{fig:tbs_cdf}
%     \end{subfigure}
% \end{figure}

% \begin{figure*}[!t]
%     \centering
%     \begin{subfigure}[b]{0.245\linewidth}
%         \centering
%         \includegraphics[width=\textwidth]{fig/oneway_dealy.pdf}
%         \caption{Oneway delay.}
%         \label{fig:tbs_cdf}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.245\linewidth}
%         \centering
%         \includegraphics[width=\textwidth]{fig/delay_loss_a.pdf}
%         \caption{Case one.}
%         \label{fig:tbs_cdf}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.245\linewidth}
%         \centering
%         \includegraphics[width=\textwidth]{fig/delay_loss_b.pdf}
%         \caption{Case two.}
%         \label{fig:tbs_cdf}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.245\linewidth}
%         \centering
%         \includegraphics[width=\textwidth]{fig/delay_loss_c.pdf}
%         \caption{Case three.}
%         \label{fig:tbs_cdf}
%     \end{subfigure}
%     \hfill
%     % \vspace{-10pt}
% \end{figure*}


% \begin{figure}[!t]
%     \centering
%     \includegraphics[width=0.98\linewidth]{fig/rcv_pkt_time_dif.pdf}
%     \caption{The difference between two consecutively received packets..}
%     \label{fig:tbs_cdf}
% \end{figure}

\subsection{Cell tower usage monitoring}

Developing systems that can achieve simultaneous high throughput and low latency communication via LTE is know to be challenging, due to the unpredictable capacity of the LTE channel. One cell tower is able to support internet connections for hundreds of mobile users. Traffic generated by mobile users vary is highly heterogeneous in terms of the data volume and vary significantly along time. On the other hand, the totally bandwidth of one cell tower is fixed and much lower compared with the Ethernet core network. As a result, the available bandwidth of the cell tower is highly unpredictable. In this section, we monitoring the traffic pattern of the cell tower in a commercial LTE network, which provides valuable insights for developing a low latency and high throughput LTE based communication system. 

\subsubsection{Traffic patter along time}

\textbf{Usage variations within one day}
\begin{figure}[!t]
    \centering
    \begin{subfigure}[b]{0.498\linewidth}
        \centering
        \includegraphics[width=\textwidth]{fig/stat_1hour_a.pdf}
        \caption{Downlink PRB usage.}
        \label{fig:2UE_1cell}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.498\linewidth}
        \centering
        \includegraphics[width=\textwidth]{fig/stat_1hour_b.pdf}
        \caption{Uplink PRB usage.}
        \label{fig:2UE_2cell}
    \end{subfigure}
    \hfill
    
    \begin{subfigure}[b]{0.49\linewidth}
        \centering
        \includegraphics[width=\textwidth]{fig/stat_1hour_c.pdf}
        \caption{Delivered downlink data.}
        \label{fig:2UE_1cell}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.49\linewidth}
        \centering
        \includegraphics[width=\textwidth]{fig/stat_1hour_d.pdf}
        \caption{Delivered uplink data.}
        \label{fig:2UE_2cell}
    \end{subfigure}
    \hfill
    
    \caption{Usage pattern of one 20MHz and one 10MHz cell tower. }
    \label{fig:UE_fairness}
    % \vspace{-10pt}
\end{figure}

\begin{figure}[!t]
    \centering
    \begin{subfigure}[b]{0.49\linewidth}
        \centering
        \includegraphics[width=\textwidth]{fig/stat_1hour_e.pdf}
        \caption{Downlink PRB usage.}
        \label{fig:2UE_1cell}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.49\linewidth}
        \centering
        \includegraphics[width=\textwidth]{fig/stat_1hour_f.pdf}
        \caption{Uplink PRB usage.}
        \label{fig:2UE_2cell}
    \end{subfigure}
    \hfill
    
    \begin{subfigure}[b]{0.49\linewidth}
        \centering
        \includegraphics[width=\textwidth]{fig/stat_1hour_g.pdf}
        \caption{Delivered downlink data.}
        \label{fig:2UE_1cell}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.49\linewidth}
        \centering
        \includegraphics[width=\textwidth]{fig/stat_1hour_h.pdf}
        \caption{Delivered uplink data.}
        \label{fig:2UE_2cell}
    \end{subfigure}
    \hfill
    
    \caption{Usage pattern of one 20MHz and one 10MHz cell tower. }
    \label{fig:UE_fairness}
    % \vspace{-10pt}
\end{figure}

Figure--1 Downlink/Uplink
sub-figure-1: x-axis 24 hours of a day; y-axis the ratio of PRB used 
sub-figure-2: x-axis 24 hours of a day; y-axis the data delivered
In each sub-figure, we have three curves: 20MHz/10MHz/5MHz cell tower 
% (\todo{Do we need to consider urban and rural area?})
 
 
% \begin{itemize}
% \item Figure--2 

% sub-figure-1: x-axis 60 minutes of one hour; y-axis the ratio of PRB used 
    
% sub-figure-2: x-axis 60 minutes of one hour; y-axis the data delivered

% In each sub-figure, we have three curves: 20MHz/10MHz/5MHz cell tower 

% \end{itemize}
\textbf{Usage variations within a short peroid of time (10s)}
\begin{figure}[!t]
    \centering
    \begin{subfigure}[b]{0.99\linewidth}
        \centering
        \includegraphics[width=\textwidth]{fig/stat_1min_a.pdf}
        \caption{Averaged busy and idle PRBs in every 100ms.}
        \label{fig:2UE_1cell}
    \end{subfigure}
    \hfill
    
    \begin{subfigure}[b]{0.99\linewidth}
        \centering
        \includegraphics[width=\textwidth]{fig/stat_1min_b.pdf}
        \caption{Total transmitted data for every 100ms.}
        \label{fig:2UE_1cell}
    \end{subfigure}
    \hfill
    \caption{PRB usage and the data delivery of a 20MHz cell tower in 60 seconds interval. }
    \label{fig:UE_fairness}
    % \vspace{-10pt}
\end{figure}

Figure--1 Down-link/Uplink
sub-figure-1: x-axis sub-frames (10s); y-axis the ratio of PRB used 
sub-figure-2: x-axis sub-frames (10s); y-axis the data delivered
In each sub-figure, we have plot the top three users that occupies most resource blocks 

sub-figure-3: x-axis sub-frames (10s); y-axis the ratio of PRB used 
sub-figure-4: x-axis sub-frames (10s); y-axis the data delivered
In each sub-figure, we have plot the top three users that has got most data from the cell tower

Is there any user that occupy significant amount of PRBs? Is there any user that delivers significant amount of data?

Figure--2 D/L (bar)
sub-figure-1: x-axis 60 minutes of one hour y-axis stacked number of prbs (top 3 users and the rest)
sub-figure-2: x-axis 60 minutes of one hour y-axis stacked number of transmitted data (top 3 users and the rest)


\textbf{How many users is observed in one minute?}
% Figure-1: D/L For each minute within one hour, how many users is observed?

Figure-1: D/L 
x-axis 60 minutes y-axis the total number of users observed in each minute -- multiple curves for multiple cell towers (5MHz, 10Mhz, 20Mhz)
Expected results: the wider the bandwidth, more user is supported.

\subsubsection{Traffic pattern for one UE running different applications}

Compare the ground truth traffic pattern (Youtube, skype, webbrowsing) of a know UE and the similar observed pattern from unknown UE. 

How to infer the applications that a UE was doing is left as future work.

\subsubsection{Traffic correlation across cell-towers}

We also investigate the traffic correlation across cell-towers that are geographically close. Due to carrier-aggregation of LTE-A standard, two cell towers with different frequencies can server one user simultaneously. Therefore, there could exists some correlation between the traffic pattern across cell towers. 

Figure --1 x-axis -- time y-axis correlation between traffice patterns across two cell towers
% \begin{figure}[!t]
%     \centering
%     \begin{minipage}[b]{0.48\linewidth}
%         \centering
%         \includegraphics[width=\textwidth]{fig/reTx_load.pdf}
%         \caption{UE received data from 1,cell; 2, cell with retransmissions removed; and 3, kernel socket.}
%         \label{fig:tbs_cdf}
%     \end{minipage}
%     \hfill
%     \begin{minipage}[b]{0.48\linewidth}
%         \centering
%         \includegraphics[width=\textwidth]{fig/reTx_ratio.pdf}
%         \caption{Ratio of 1,retransmitted data; 2, retransmitted TB; and 3, transmitted overhead.}
%         \label{fig:prb_cdf}
%     \end{minipage}
%     \hfill
%     % \vspace{-10pt}
% \end{figure}

% \begin{figure}[!t]
%     \centering
%     \begin{subfigure}[b]{0.48\linewidth}
%         \centering
%         \includegraphics[width=\textwidth]{fig/mcs_cdf_1.pdf}
%         \caption{The first spatial stream with offered load 11 Mbps.}
%         \label{fig:tbs_cdf}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.48\linewidth}
%         \centering
%         \includegraphics[width=\textwidth]{fig/mcs_cdf_2.pdf}
%         \caption{The second spatial stream with offered load 11 Mbps.}
%         \label{fig:prb_cdf}
%     \end{subfigure}
%     \hfill
    
%     \centering
%     \begin{subfigure}[b]{0.48\linewidth}
%         \centering
%         \includegraphics[width=\textwidth]{fig/mcs_cdf_3.pdf}
%         \caption{The first spatial stream with offered load 27 Mbps.}
%         \label{fig:tbs_cdf}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.48\linewidth}
%         \centering
%         \includegraphics[width=\textwidth]{fig/mcs_cdf_4.pdf}
%         \caption{The second spatial stream with offered load 27 Mbps.}
%         \label{fig:prb_cdf}
%     \end{subfigure}
%     \hfill
    
%     \caption{MCS distribution for all transmitted TB and retransmitted TB, when offered load 11 Mbps and 27 Mbps. }
%     \label{fig:UE_fairness}
%     % \vspace{-10pt}
% \end{figure}

% \begin{figure}[!t]
%     \centering
%     \begin{minipage}[b]{0.48\linewidth}
%         \centering
%         \includegraphics[width=\textwidth]{fig/tbs_cdf.pdf}
%         \caption{CDF of transmitted data in each subframe.}
%         \label{fig:tbs_cdf}
%     \end{minipage}
%     \hfill
%     \begin{minipage}[b]{0.48\linewidth}
%         \centering
%         \includegraphics[width=\textwidth]{fig/prb_cdf.pdf}
%         \caption{CDF of allocated PRB in each subframe.}
%         \label{fig:prb_cdf}
%     \end{minipage}
%     \hfill
%     % \vspace{-10pt}
% \end{figure}

\subsection{LTE-A resource allocation}

\begin{figure*}
%\vspace{-12pt}
  \begin{minipage}[t]{0.32\linewidth}
      \centering
      \includegraphics[width=0.99\linewidth]{fig/CarrierAggregation.pdf}
      \caption{Carrier aggregation in LTE Advanced. The UE is associated with a priminary serving cell. The neighbouring cell towers can also be used to transmit data to the UE when necessary.}
      \label{fig:CA}
  \end{minipage}\hfill
  \begin{minipage}[t]{0.32\linewidth}
     \centering
     \includegraphics[width=0.98\linewidth]{fig/UE_rx_rate.pdf}
      \caption{The UE received data rate from 1, kernel socket; 2, the associated cell (5MHz); 3, a neighbouring cell (20MHz) 4, the aggregated rate from 2 cells.}
      \label{fig:UE_rx_rate}
   \end{minipage}\hfill
   \begin{minipage}[t]{0.32\linewidth}
     \centering
     \includegraphics[width=0.98\linewidth]{fig/ue_rx_data.pdf}
      \caption{The UE received data from 1, kernel socket; 2, the associated cell (5MHz); 3, a neighbouring cell (20MHz) 4, the aggregation of 2 cells.}
      \label{fig:UE_rx_rate}
   \end{minipage}
\end{figure*}


% \begin{figure}[h]
%   \begin{center}
%       \includegraphics[width=0.8\linewidth]{fig/CarrierAggregation.pdf}
%       \caption{Carrier aggregation in LTE Advanced. The UE is associated with a priminary serving cell. The neighbouring cell towers can also be used to transmit data to the UE when necessary.}
%       \label{fig:CA}
%   \end{center}
%   \vspace{-15pt}
% \end{figure} 

Different from LTE where one UE only talks with one cell tower at a time, LTE Advanced allows the UE to talk to multiple cell towers simultaneously, which is referred to as Carrier Aggregation. Therefore, the resource allocations schemes running on each cell tower must share information among each other. The final allocation decision must be derived based on the local traffic demand and the global information shared between cell towers. We investigate how the cell tower handles the allocation under different scenarios.

\textbf{Experiment methodology.} We set up an AWS server and build a UDP connection between our UE and the server. The server transmits the same amount data to the UE with different data rate. We measure 1, the data rate received by the UE; 2, how many data are delivered from the primary serving cell tower to the UE. 


\textbf{When will the Carrier Aggregation be triggered?}
% \begin{figure}[h]
%   \begin{center}
%       \includegraphics[width=0.98\linewidth]{fig/UE_rx_rate.pdf}
%       \caption{The UE received data rate from 1, kernel socket; 2, the associated cell (5MHz); 3, a neighbouring cell (20MHz) 4, the aggregated rate from 2 cells.}
%       \label{fig:UE_rx_rate}
%   \end{center}
% \end{figure} 

% \begin{figure}[h]
%   \begin{center}
%       \includegraphics[width=0.98\linewidth]{fig/ue_rx_data.pdf}
%       \caption{The UE received data from 1, kernel socket; 2, the associated cell (5MHz); 3, a neighbouring cell (20MHz) 4, the aggregated rate from 2 cells.}
%       \label{fig:UE_rx_rate}
%   \end{center}
% \end{figure} 
Figure-1: x-axis Server Offered Load (Mbits/sec) ; y-axis is UE received data (Mbits/sec). We also plot the theoretical data rate that the cell tower can support. We can calculate the theoretical data rate since we know the bandwidth and we also know the MCS. 

Expected results: the received data rate can catch up with the transmitted data rate, even when the transmitted data rate is larger then the theoretical upper bound that the cell tower can support.

Figure-2: x-axis server transmit data rate; y-axis the amount of data delivered from the primary serving cell to the UE

Expected results: When data rate is high, only a portion of the data are delivered from the associated cell tower. 

\textbf{Is the missing data delivered by other cell towers?}

Figure-1: x-axis index of the sub-frames y-axis: total resource blocks used by the UE from 2 cell towers (stacked individual resource blocks from each tower)

Figure-2: x-axis index of the sub-frames y-axis: data delivered to the UE from 2 cell towers (stacked)

Questions to answer: when does secondary serving cell begin to deliver data to the UE? In the middle of the transmission or from the beginning?


\begin{figure}[!t]
    \centering
    \begin{subfigure}[b]{0.97\linewidth}
        \centering
        \includegraphics[width=\textwidth]{fig/OneUE_prb.pdf}
        \caption{Averaged allocated PRBs for UE from two cells.}
        \label{fig:2UE_1cell}
    \end{subfigure}
    \hfill
    
    \begin{subfigure}[b]{0.97\linewidth}
        \centering
        \includegraphics[width=\textwidth]{fig/OneUE_tbs.pdf}
        \caption{Total received data in 10ms by UE from two cells.}
        \label{fig:2UE_2cell}
    \end{subfigure}
    \hfill
    
    \begin{subfigure}[b]{0.97\linewidth}
        \centering
        \includegraphics[width=\textwidth]{fig/OneUE_rtt.pdf}
        \caption{Oneway delay of the received packets.}
        \label{fig:2UE_1cell}
    \end{subfigure}

    
    \caption{Usage pattern of one 20MHz and one 10MHz cell tower. }
    \label{fig:UE_fairness}
    % \vspace{-10pt}
\end{figure}
\textbf{How does the carrier aggregation affects the delay since the packets could arrive from different cell towers.}

Figure-1: x-axis packet index y-axis packet one way delay

Analyzing how does the carrier aggregation affects the one way delay. 

\textbf{Is current TCP aware of this and can make use of this?}

We measure the performance of CUBIC algorithm and see whether CUBIC will trigger the carrier aggregation or not. 

Figure-1: three sub-figures

sub-figure-1: x-axis time, y-axis CUBIC throughput 

sub-figure-2: x-axis prb or throughput of cell tower 1

sub-figure-3: x-axis prb or throughput of cell tower 2

\textbf{How would the hand over affect the transmission?}

Do we need hand over in LTE-A anymore? Does it affect the transmission? 
Figure-1: three sub-figures

sub-figure-1: x-axis time, y-axis CUBIC throughput 

sub-figure-1: x-axis time, y-axis CUBIC oneway delay 

\subsubsection{The fairness between UEs}

\begin{figure}[!t]
    \centering
    \begin{subfigure}[b]{0.49\linewidth}
        \centering
        \includegraphics[width=\textwidth]{fig/CA_2UE_a.pdf}
        \caption{Two UE associated with one cell tower.}
        \label{fig:2UE_1cell}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.49\linewidth}
        \centering
        \includegraphics[width=\textwidth]{fig/CA_2UE_b.pdf}
        \caption{Two UE associated with two dfferent cell tower.}
        \label{fig:2UE_2cell}
    \end{subfigure}
    \hfill
    \caption{How would the LTE network handles two UE associated with 1, the same cell tower; 2, two cell towers that geographically close to each other. }
    \label{fig:UE_fairness}
    % \vspace{-10pt}
\end{figure}

\textbf{Experiment methodology.} We build two UDP connections between two UE and two separate servers. The server sends data to the UE with different transmission rate. We investigate how the LTE network allocates bandwidth for these two UEs. 

\textbf{Two co-located mobile phones-- associated with the same cell tower.}

Figure-1: four subfigures

Subfigure1: x-axis Tx data rate of UE2 y-axis TX data rate of UE1 color the PRB allocated for UE1 -- all data are collected from cell 1

Subfigure2: x-axis Tx data rate of UE2 y-axis TX data rate of UE1 color the PRB allocated for UE2 -- all data are collected from cell 1

Subfigure3: x-axis Tx data rate of UE2 y-axis TX data rate of UE1 color the PRB allocated for UE1 -- all data are collected from cell 2

Subfigure4: x-axis Tx data rate of UE2 y-axis TX data rate of UE1 color the PRB allocated for UE2 -- all data are collected from cell 2

\textbf{One mobile phones close to the cell tower and one far away-- associated with the same cell tower.}
The same figure as above.


Another interesting question is that, how would the traffic from the secondary serving cell affects the bandwidth allocation schemes in the primary serving cell? Just as Figure~\ref{fig:2UE_2cell} shows, if UE-1 and UE-2 both are communicating with their own associated cell tower with high data rate, will the LTE network use carrier aggregation? If yes, how would LTE handles the fairness?
\textbf{Two co-located mobile phones-- associated with the same cell tower.}

Figure-1: four subfigures

Subfigure1: x-axis Tx data rate of UE2 y-axis TX data rate of UE1 color the PRB allocated for UE1 -- all data are collected from cell 1

Subfigure2: x-axis Tx data rate of UE2 y-axis TX data rate of UE1 color the PRB allocated for UE2 -- all data are collected from cell 1

Subfigure3: x-axis Tx data rate of UE2 y-axis TX data rate of UE1 color the PRB allocated for UE1 -- all data are collected from cell 2

Subfigure4: x-axis Tx data rate of UE2 y-axis TX data rate of UE1 color the PRB allocated for UE2 -- all data are collected from cell 2

\textbf{One mobile phones close to the cell tower and one far away-- associated with the same cell tower.}
The same figure as above.

\subsubsection{The fairness between traffic}

How does the LTE network handles the scenario where high throughput traffic, such as TCP downloading and low latency traffic, such as skype, coexists with each other? 





==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.75.  \country is now obligatory for addresses.
	       Added \AtBeginMaketitle

Version 1.76.  Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.77.  Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.78.  Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.79.  Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.80.  New journals: DLT, FAC

